Breaking the Familiarity Bias: Employing Virtual Reality Environments to Enhance Team Formation and Inclusion

Team closeness provides the foundations of trust and communication, contributing to teams' success and viability. However, newcomers often struggle to be included in a team since incumbents tend to interact more with other existing members. Previous research suggests that online communication technologies can help team inclusion by mitigating members' perceived differences. In this study, we test how virtual reality (VR) can promote team closeness when forming teams. We conducted a between-subject experiment with teams working in-person and VR, where two members interacted first, and then a third member was added later to conduct a hidden-profile task. Participants evaluated how close they felt with their teammates after the task was completed. Our results show that VR newcomers felt closer to the incumbents than in-person newcomers. However, incumbents' closeness to newcomers did not vary across conditions. We discuss the implications of these findings and offer suggestions for how VR can promote inclusion.

==> tables/mixed_model_familiarity.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{lccccc}
  \hline
 & Estimate & Std. Error & d.f. & \textit{t} value & Pr($>$$|$t$|$) \\ 
  \hline
  \textbf{Fixed Effects} & & & & & \\
  Intercept & -0.11 & 0.20 & 24.05 & -0.54 & 0.59 \\ 
  (H3) Condition (1: VR) & -0.29 & 0.26 & 28.11 & -1.12 & 0.27 \\ 
  Gender Homophily & 0.48$\dagger$ & 0.27 & 29.15 & 1.80 & 0.08 \\ 
  Relative Similarity Score & 0.80** & 0.26 & 49.51 & 3.03 & 0.00 \\ 
  Support by the Environment & 0.01 & 0.13 & 46.51 & 0.11 & 0.91 \\ 
  Comm. Effectiveness & 0.17 & 0.20 & 48.78 & 0.85 & 0.40 \\ 
  Information Exchange & -0.07 & 0.17 & 48.90 & -0.40 & 0.69 \\ 
  Condition $\times$ Relative Similarity Score & -0.53$\dagger$ & 0.27 & 49.38 & -1.96 & 0.06 \\ 
  \textbf{Random Effects} & & & & & \\
  Intercept (Variance) & 0.07 & 0.26 & & & \\
  Residual (Variance) & 0.66 & 0.81 & & & \\
   \hline
\end{tabular}
\caption{Mixed-effects linear regression model estimating incumbents' familiarity bias. Number of Observations: 58. Groups (i.e., Sessions): 29. Significance codes: $\dagger p < .10$,  * $p < .05$, ** $p < .01$, *** $p < .001$}
\label{tab:mixed-effect-familiarity}
\end{table}
